Bounding the Lagrangian Hofer metric via barcodes

We provide an upper bound on the Lagrangian Hofer distance between equators in the cylinder in terms of the barcode of persistent Floer homology. The bound consists of a weighted sum of the lengths of the finite bars and the spectral distance.

==> questions.tex <==
\begin{enumerate}
    \item Combinatorial proof for $\beta_1 \leq \gamma$?
    \item Is the bound optimal?
    \item Is the bound comparable to Khanevsky's bound?
    \item $\gamma(L,L_0)$ is bounded while $d_H(L,L_0)$ is not.
    Is there an unbounded lower bound of $d_H(L,L_0)$ in terms of the
    barcode? Maybe $\sum_{i=1}^n \beta_i(L,L_0)$?
    \item The sum $\sum 2^i \beta_i$ looks odd. Does this measurement have a ``more conceptual" motivation?
\end{enumerate}
